Efficient Personalized Speech Enhancement through Self-Supervised Learning

This work presents self-supervised learning methods for developing monaural speaker-specific (i.e., personalized) speech enhancement models. While generalist models must broadly address many speakers, specialist models can adapt their enhancement function towards a particular speaker's voice, expecting to solve a narrower problem. Hence, specialists are capable of achieving more optimal performance in addition to reducing computational complexity. However, naive personalization methods can require clean speech from the target user, which is inconvenient to acquire, e.g., due to subpar recording conditions. To this end, we pose personalization as either a zero-shot task, in which no additional clean speech of the target speaker is used for training, or a few-shot learning task, in which the goal is to minimize the duration of the clean speech used for transfer learning. With this paper, we propose self-supervised learning methods as a solution to both zero- and few-shot personalization tasks. The proposed methods are designed to learn the personalized speech features from unlabeled data (i.e., in-the-wild noisy recordings from the target user) without knowing the corresponding clean sources. Our experiments investigate three different self-supervised learning mechanisms. The results show that self-supervised models achieve zero-shot and few-shot personalization using fewer model parameters and less clean data from the target user, achieving the data efficiency and model compression goals.

==> tables/tbl_ablation.tex <==
\begin{table}[ht!]
\centering
\caption{Ablation study on contrastive mixtures.}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lccrr}\toprule
\textbf{Model}
& \textbf{$\lambda_p$}
& \textbf{$\lambda_n$}
& \textbf{\makecell[r]{\# of examples}}
& \textbf{\makecell[r]{SI-SDRi}} \\
\midrule
\multirow{4}{*}[0pt]{GRU Large} % -7pt
& 0 & 0 
\\ % \cmidrule{2-5}
& 1 & 0
\\ % \cmidrule{2-5}
& 0 & 1
\\ % \cmidrule{2-5}
& 1 & 1
\\
\midrule
\multirow{4}{*}[0pt]{GRU Medium} % -7pt
& 0 & 0 
\\ % \cmidrule{2-5}
& 1 & 0
\\ % \cmidrule{2-5}
& 0 & 1
\\ % \cmidrule{2-5}
& 1 & 1
\\
\midrule
\multirow{4}{*}[0pt]{GRU Small} % -7pt
& 0 & 0 
\\ % \cmidrule{2-5}
& 1 & 0
\\ % \cmidrule{2-5}
& 0 & 1
\\ % \cmidrule{2-5}
& 1 & 1
\\
\bottomrule
\end{tabular}
\label{tab:datasets}
\end{table}

==> tables/tbl_corpora.tex <==
\begin{table}[t]
\centering
\caption{Glossary of experiment corpora and notations.}
\renewcommand{\arraystretch}{1.2}
\begin{tabularx}{\columnwidth}{LLclR}
% \begin{tabular}{lllr}
\toprule
\textbf{Corpus}
% & \textbf{Subset}
& \textbf{Quantity}
&
& \textbf{Set}
& \textbf{Duration}
\\
\midrule
\multirow{7}{*}{\makecell[l]{LibriSpeech \\ \cite{PanayotovV2015Librispeech} }}
% & \multirow{5}{*}{\makecell[l]{\textit{train-clean-100}}}
& \multirow{5}{*}{\makecell[l]{\num{20} spkrs}}
& \multirow{5}{*}{\makecell[l]{\includegraphics[scale=0.5]{figures/icon_ss.pdf}}}
& $\SSpretrain$
& \SI{22.5}{\min\per\spkr}
\\
% &
&&& $\SSpreval$
& \SI{30}{\sec\per\spkr}
\\
% &
&&& $\SStrain$
& \SI{60}{\sec\per\spkr}
\\
% &
&&& $\SSval$
& \SI{30}{\sec\per\spkr}
\\
% &
&&& $\SStest$
& \SI{30}{\sec\per\spkr}
\\ \cmidrule{2-5}
% & \textit{train-clean-360}
& \num{1132} spkrs
& \multirow{2}{*}{\makecell[l]{\includegraphics[scale=0.5]{figures/icon_sa.pdf}}}
& $\SAtrain$
& \SI{443}{\hour}
\\
% & \textit{train-clean-100}
& \num{20} spkrs
&& $\SAval$
& \SI{8}{\hour}
\\
\midrule
\multirow{2}{*}{\makecell[l]{\makecell{FSD50K \\ \cite{FonsecaE2020fsd50k}}}}
% & \multirow{2}{*}{\makecell[l]{\textit{eval\_audio}}}
& \num{13,339} noises
& \multirow{2}{*}{\makecell[l]{\includegraphics[scale=0.5]{figures/icon_m.pdf}}}
& $\Mtrain$
& \SI{48}{\hour}
\\
% &
& \num{1929} noises
&& $\Mval$
& \SI{7}{\hour}
\\ 
% % \cmidrule{2-4}
% % % % % ASWIN NOTE: This corpus does exist but isn't used in the experiment.
% % & \textit{dev\_audio}
% & \num{5298} noises
% & \Ntrain
% & \SI{20}{\hour}
% \\
\midrule
\multirow{3}{*}{\makecell[l]{\makecell{MUSAN\\ \cite{SnyderD2015MUSAN}}}}
% & \multirow{2}{*}{\makecell[l]{\textit{free-sound}}}
& \num{616} noises
& \multirow{3}{*}{\makecell[l]{\includegraphics[scale=0.5]{figures/icon_n.pdf}}}
& $\Ntrain$
& \SI{5}{\hour}
\\
% &
& \num{60} noises
&& $\Nval$
& \SI{0.5}{\hour}
\\
% & \textit{sound-bible}
& \num{61} noises
&& $\Ntest$
& \SI{0.3}{\hour}
\\
\bottomrule
\end{tabularx}
% \end{tabular}
\label{tab:datasets}
\end{table}

==> tables/tbl_methods.tex <==
\begin{table}[t]

\newcommand\cw{3.3in} % equation column width
\centering
\caption{Overview of pre-training procedures for\\personalized speech enhancement models.}
\label{tab:equations}
\raggedright{

\setlength{\tabcolsep}{2pt}
\def\arraystretch{1.5}
\begin{tabular}{m{1ex}m{4pt}m{\cw}m{1in}}
\multicolumn{4}{l}{
\textbf{Generalist Pre-Training} (Fully-Supervised)
} \\
\multirow{3}{*}{\rotatebox[origin=c]{90}{SE}}
& \multirow{3}{*}{\color{tab_gray}\vline height 42pt depth 0pt width 2pt}
& $\bm{x}=\bm{s}+\bm{n} ; \quad \bm{s} \in \mathbb{G}_{\text{tr}}, \bm{n} \in \mathbb{N}_{\text{tr}}$ \\
&& $\bm{y}=f_{\text{SE}}\left(\bm{x} ; \mathcal{W}_{\text{SE}}\right)$ \\
&& \inlineequation[eq:loss_baseline]{
\mathcal{L}_{\text{SE}} = \dist{\bm{y}}{\bm{s}}
}
\end{tabular}\\[1em]

\begin{tabular}{m{1ex}m{4pt}m{\cw}m{1in}}
\multicolumn{4}{l}{
\textbf{Premixture} (Simulation of sampling from $\SSnpretrain$)
} \\
&& \inlineequation[eq:premixture]{
\tilde{\bm{s}} = \bm{s} + \bm{m}; \quad \bm{s}\in \SSpretrain, \hspace{2mm} \bm{m} \in \Mtrain}
\end{tabular}\\[1em]

\begin{tabular}{m{1ex}m{4pt}m{\cw}m{1in}}
\multicolumn{4}{l}{
\textbf{Specialist Pre-Training} (Self-Supervised / ZSL)
} \\
\multirow{3}{*}{\rotatebox[origin=c]{90}{\textcolor{tab_blue}{PseudoSE}}}
& \multirow{3}{*}{\color{tab_blue}\vline height 42pt depth 0pt width 2pt}
& $\tilde{\bm{x}} = \tilde{\bm{s}} + \bm{n}; \quad \tilde{\bm{s}}\in\tilde{\mathbb{S}}_\text{\textbf{p}-tr},\hspace{2mm}\bm{n}\in\Ntrain$
\\
&& $\tilde{\bm{y}} = f_\text{PSE}(\tilde{\bm{x}}; \mathcal{W}_\text{PSE})$
\\
&& \inlineequation[eq:obj_pseudose]{
\mathcal{L}_\text{PSE} = \dist{\tilde{\bm{y}}}{\tilde{\bm{s}}}} \\[1em]

\multirow{11}{*}{\rotatebox[origin=c]{90}{\textcolor{tab_green}{Contrastive Mixtures}}}
& \multirow{11}{*}{\color{tab_green}\vline height 162pt depth 0pt width 2pt}
& $\tilde{\bm{x}}_1^\oplus = \tilde{\bm{s}}^\oplus + \bm{n}_1; \quad \tilde{\bm{s}}^\oplus \in \tilde{\mathbb{S}}_\text{\textbf{p}-tr}, \hspace{2mm} \bm{n}_1, \bm{n}_2 \in \Ntrain$
\\
&& $\tilde{\bm{x}}_2^\oplus = \tilde{\bm{s}}^\oplus + \bm{n}_2$
\\
&& $\tilde{\bm{x}}_1^\ominus = \tilde{\bm{s}}^\ominus_1 + \bm{n}; \quad \tilde{\bm{s}}^\ominus_1, \tilde{\bm{s}}^\ominus_2 \in \tilde{\mathbb{S}}_\text{\textbf{p}-tr}, \hspace{2mm} \bm{n} \in \Ntrain$
\\
&& $\tilde{\bm{x}}_2^\ominus = \tilde{\bm{s}}^\ominus_2 + \bm{n}$
\\
&& $\tilde{\bm{y}}_1^\oplus = f_\text{CM}(\tilde{\bm{x}}_1^\oplus; \mathcal{W}_\text{CM})$
\\
&& $\tilde{\bm{y}}_2^\oplus = f_\text{CM}(\tilde{\bm{x}}_2^\oplus; \mathcal{W}_\text{CM})$
\\
&& $\tilde{\bm{y}}_1^\ominus = f_\text{CM}(\tilde{\bm{x}}_1^\ominus; \mathcal{W}_\text{CM})$
\\
&& $\tilde{\bm{y}}_2^\ominus = f_\text{CM}(\tilde{\bm{x}}_2^\ominus; \mathcal{W}_\text{CM})$
\\
&& \inlineequation[eq:loss_positive]{\mathcal{L}_p =
    \mathcal{E}(\tilde{\bm{s}}^\oplus||\tilde{\bm{y}}_1^\oplus) + \mathcal{E}(\tilde{\bm{s}}^\oplus||\tilde{\bm{y}}_2^\oplus) +
    \lambda_p \big[\mathcal{E}(\tilde{\bm{y}}_1^\oplus||\tilde{\bm{y}}_2^\oplus)\big]
} \\
&& \inlineequation[eq:loss_negative]{\mathcal{L}_n = 
\mathcal{E}(\tilde{\bm{s}}_1^\ominus||\tilde{\bm{y}}_1^\ominus)
+ \mathcal{E}(\tilde{\bm{s}}_2^\ominus||\tilde{\bm{y}}_2^\ominus)
+ \lambda_n \big[\mathcal{E}(\tilde{\bm{s}}_1^\ominus||\tilde{\bm{s}}_2^\ominus)
- \mathcal{E}(\tilde{\bm{y}}_1^\ominus||\tilde{\bm{y}}_2^\ominus)\big]^2
} \\
&& \inlineequation[eq:loss_cm]{
\mathcal{L}_\text{CM} = \Bigg[ \sum_{i=1}^T\mathcal{L}_p(t) + \sum_{i=1}^T\mathcal{L}_n(t) \Bigg]} \\
% && $\displaystyle\mathcal{W}_\text{CM} \leftarrow \argmin_{\mathcal{W}_\text{CM}} \mathcal{L}_\text{CM}$
\end{tabular}\\[1em]

\begin{tabular}{m{1ex}m{4pt}m{\cw}m{1in}}
\multicolumn{4}{l}{
\textbf{Specialist Fine-Tuning} (Fully-Supervised / FSL)
} \\
&&
$\mathcal{W} \leftarrow $ Pre-Trained Weights (either 
$\mathcal{W}_\text{SE},
\mathcal{W}_\text{PSE}, \text{or }
\mathcal{W}_\text{CM}$)
\\
& \multirow{3}{*}{\color{tab_orange}\vline height 46pt depth 0pt width 2pt}
% & $\mathcal{W} \leftarrow \text{Pre-Trained Weights (either }
% \mathcal{W}_\text{SE},
% \mathcal{W}_\text{PSE}, \text{ or }
% \mathcal{W}_\text{CM}
% \text{)}$
% \\
& $\bm{x} = \bm{s}+\bm{n} ; \quad \bm{s} \in \SStrain, \bm{n} \in \Ntrain$
\\
&& $\bm{y} = f(\bm{x} ; \mathcal{W})$
\\
% && \inlineequation[eq:obj_finetuning]{
% \mathcal{W} \leftarrow \argmin_{\mathcal{W}} \dist{\bm{y}}{\bm{s}}}
% && $\mathcal{L}_{\text{SE}} = \dist{\bm{y}}{\bm{s}}$
&& \inlineequation[eq:ft_fsl]{\displaystyle\mathcal{W} \leftarrow \argmin_{\mathcal{W}} \dist{\bm{y}}{\bm{s}}}
\end{tabular}
}
\end{table}

==> tables/tbl_notation.tex <==
\begin{table*}[ht]
\centering
\caption{Glossary of dataset notation.}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llll}\toprule
& \textbf{Set}
& \textbf{Subsets}
& \textbf{Description}
\\
\midrule
\makecell[l]{\includegraphics[scale=0.5]{figures/icon_sa.pdf}}
& $\SAfull$
& $\SAtrain / \SAval$
& Clean speech from many other speakers
\\ \cmidrule{2-4}
\makecell[l]{\includegraphics[scale=0.5]{figures/icon_ss.pdf}}
& $\SSfull$
&
& Hypothetical set of all utterances from target speaker
\\
&& $\SSnpretrain / \SSnpreval$
& Target's noisy speech (corrupted by $\Mfull$), referred to as the set of \textit{premixture} data
\\
&& $\SStrain / \SSval$
& Target's provided clean speech (only available in FSL context)
\\
&& $\SStest$
& Set-aside speaker-specific clean speech used only for objective model evaluation
\\ \cmidrule{2-4}
\makecell[l]{\includegraphics[scale=0.5]{figures/icon_m.pdf}}
& $\Mfull$
& $\Mtrain / \Mval$
& \makecell[l]{Premixture noises corrupting the majority of target speaker's utterances;\\
on its own, inaccessible to the service provider for model training}
\\ \cmidrule{2-4}
\makecell[l]{\includegraphics[scale=0.5]{figures/icon_n.pdf}}
& $\Nfull$
& $\Ntrain / \Nval$
& Injection noises used by service provider for model training
\\
&& $\Ntest$
& Set-aside unseen injection noises used only for objective model evaluation
\\
\bottomrule
\end{tabular}
\label{tab:glossary}
\end{table*}

==> tables/tbl_notation_verbose.tex <==
\begin{table*}[ht]
\centering
\caption{Glossary of dataset notation.}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{lM{2.5in}lM{3in}}\toprule
\textbf{Set}
& \textbf{Description}
& \textbf{Subset}
& \textbf{Description}
\\
\midrule
\multirow{2.4}{*}{\makecell[l]{
$\SAfull$}}
& \multirow{2.4}{2.3in}{Large set containing utterances from many different speakers}
& $\SAtrain$
& Training set
\\ \cmidrule{3-4}
&& $\SAval$
& Validation set
\\
\midrule
\multirow{10}{*}{\makecell[l]{
$\SSfull$}}
& \multirow{10}{2.3in}{Small set containing utterances only from the ``personalization target'' or ``test-time speaker''}
& $\SSpretrain$
& Training set used for pre-training; we assume it is contaminated by $\Mtrain$, therefore the enhancement models can only utilize the resulting noisy observations:  $\tilde{\mathbb{S}}_\text{tr}$
\\ \cmidrule{3-4}
&& $\SSpreval$
& Validation set used for pre-training; we assume it is contaminated by $\Mval$, therefore the enhancement models can only utilize the resulting noisy observations:  $\tilde{\mathbb{S}}_\text{vl}$
\\ \cmidrule{3-4}
&& $\SStrain$
& Training set used for fine-tuning; in the FSL context, the test-time provides a small amount of recordings which are known to be noise-free
\\ \cmidrule{3-4}
&& $\SSval$
& Validation set used for fine-tuning in the FSL context
\\ \cmidrule{3-4}
&& $\SStest$
& Speaker-specific test set used to evaluate the personalized enhancement performance of both generalist and specialist models
\\
\midrule
\multirow{2.4}{*}{\makecell[l]{
$\Mfull$}}
& \multirow{2.4}{2.3in}{Large set of premixture noise signals, which represent the test-time speaker's environment}
& $\Mtrain$
& Training set
\\ \cmidrule{3-4}
&& $\Mval$
& Validation set
\\
\midrule
\multirow{3.5}{*}{\makecell[l]{
$\Nfull$}}
& \multirow{3.5}{2.3in}{Large set of injection noise signals which are known to the model, i.e., used to create artificial mixtures for supervised machine learning}
& $\Ntrain$
& Training set
\\ \cmidrule{3-4}
&& $\Nval$
& Validation set
\\ \cmidrule{3-4}
&& $\Ntest$
& Test set, injected onto $\SStest$ for evaluating models
\\
\bottomrule
\end{tabular}
\label{tab:glossary}
\end{table*}

==> tables/tbl_results.tex <==
\begin{table*}[ht!]
\centering
\caption{SI-SDR improvement from generalist and specialist GRU models.}
\begin{tabular}{llrrrrr}
\toprule
   \multirow{2}{*}{\textbf{Model Size}}
 & \multirow{2}{*}{\textbf{Training Configuration}}
 & \textbf{No-Shot}
 & \multicolumn{3}{c}{\textbf{Few-Shot (Fine-Tuning)}}
 \\\cmidrule(lr){3-3} \cmidrule(lr){4-6}
 &
 & $T=\SI{0}{\second}$
 & $T=\SI{5}{\second}$
 & $T=\SI{10}{\second}$
 & $T=\SI{30}{\second}$ \\\midrule
\multirow{5}{*}{Small}
 & Generalist
 & \num{7.441}  & \num{7.875}   & ---   & ---   \\ \cmidrule{2-2}
 & Specialist
 & \num{7.372}  & ---    & ---   & ---   \\
 & Specialist w/ Contrastive Loss
 & \num{7.847}  & ---    & ---   & ---   \\
 & Specialist w/ Purified Loss
 & \num{7.651}  & ---    & ---   & ---   \\
 & Specialist w/ Contrastive + Purified Loss
 & \num{8.015}  & ---    & ---   & ---   \\
\midrule
\multirow{5}{*}{Medium}
 & Generalist
 & \num{8.550}  & \num{8.964}   & ---   & ---   \\ \cmidrule{2-2}
 & Specialist
 & \num{7.665}  & ---    & ---   & ---   \\
 & Specialist w/ Contrastive Loss
 & \num{8.401}  & ---    & ---   & ---   \\
 & Specialist w/ Purified Loss
 & \num{8.040}  & ---    & ---   & ---   \\
 & Specialist w/ Contrastive + Purified Loss
 & \num{8.591}  & ---    & ---   & ---   \\
 \midrule
\multirow{5}{*}{Large}
 & Generalist
 & \num{9.042}  & \num{9.440}   & ---   & ---   \\ \cmidrule{2-2}
 & Specialist
 & \num{8.265}  & ---    & ---   & ---   \\
 & Specialist w/ Contrastive Loss
 & \num{8.622}  & ---    & ---   & ---   \\
 & Specialist w/ Purified Loss
 & \num{8.217}  & ---    & ---   & ---   \\
 & Specialist w/ Contrastive + Purified Loss
 & \num{8.778}  & ---    & ---   & ---   \\
\bottomrule
\end{tabular}
\label{tab:results}
\end{table*}

\begin{table*}[ht!]
\centering
\caption{Comparison of DPRNN-TasNet denoising models based on SI-SNR improvement.}
\begin{tabular}{lclrrrrrr}\toprule
\multirow{2}{*}{\textbf{Model Size}} 
 & \multirow{2}{*}{\textbf{Causal}}
 & \multirow{2}{*}{\textbf{Training Configuration}}
 & \multicolumn{2}{c}{\textbf{Test Context}}
 &  \multicolumn{4}{c}{\textbf{Fine-Tuning ({\sc 1S+MN})}} \\\cmidrule(lr){4-5} \cmidrule(lr){6-9}
 &
 &
 & \textsc{1S+1N} & \textsc{1S+MN}
 & $T=\SI{3}{\second}$
 & $T=\SI{5}{\second}$
 & $T=\SI{10}{\second}$
 & $T=\SI{60}{\second}$ \\\midrule
\multirow{5}{*}{\makecell[l]{
Small\\
(\SI{793}{\kilo\nothing} params.)\\
{\tiny$N=512$, $L=16$,}\\[-1ex]
{\tiny$B=128$, $H=512$,}\\[-1ex]
{\tiny$Sc=128$, $P=3$,}\\[-1ex]
{\tiny$X=8$, $R=1$}
}}
 & \multirow{5}{*}{\makecell[c]{\no}}
 & Generalist
 & 1.0 & 2.0 & --- & --- \\
 &
 & Specialist
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Contrastive Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Purified Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Contrastive + Purified Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
\midrule
\multirow{5}{*}{\makecell[l]{
Medium\\
(\SI{1.39}{\mega\nothing} params.)\\
{\tiny$\ldots$, $R=2$}
}}
 & \multirow{5}{*}{\makecell[c]{\no}}
 & Generalist
 & 1.0 & 2.0 & --- & --- \\
 &
 & Specialist
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Contrastive Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Purified Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Contrastive + Purified Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 \midrule
\multirow{5}{*}{\makecell[l]{
Large\\
(\SI{1.98}{\mega\nothing} params.)\\
{\tiny$\ldots$, $R=3$}
}}
 & \multirow{5}{*}{\makecell[c]{\no}}
 & Generalist
 & 1.0 & 2.0 & --- & --- \\
 &
 & Specialist
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Contrastive Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Purified Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Contrastive + Purified Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
\bottomrule
\end{tabular}
\label{tab:results}
\end{table*}



\begin{table*}[ht!]
\centering
\caption{Comparison of various denoising models based on SI-SNR improvement.}
\begin{tabular}{cllrrrrrr}\toprule
 \multirow{2}{*}{\textbf{Model}} 
 & \multirow{2}{*}{\textbf{Model Size}} 
 & \multirow{2}{*}{\textbf{Training Configuration}}
 & \multicolumn{2}{c}{\textbf{Test Context}}
 &  \multicolumn{4}{c}{\textbf{Fine-Tuning ({\sc 1S+MN})}} \\\cmidrule(lr){4-5} \cmidrule(lr){6-9}
 &
 &
 & \textsc{1S+1N} & \textsc{1S+MN}
 & $T=\SI{3}{\second}$
 & $T=\SI{5}{\second}$
 & $T=\SI{10}{\second}$
 & $T=\SI{60}{\second}$ \\\midrule
\multirow{15}{*}{\makecell[l]{
Conv-TasNet}}
 & \multirow{5}{*}{\makecell[l]{
Small\\
(\SI{1.76}{\mega\nothing} params.)
}}
 & Generalist
 & 1.0 & 2.0 & --- & --- \\
 &
 & Specialist
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Contrastive Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Purified Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Contrastive + Purified Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
\cmidrule(lr){2-9}
 & \multirow{5}{*}{\makecell[l]{
Medium\\
(\SI{3.37}{\mega\nothing} params.)
}}
 & Generalist
 & 1.0 & 2.0 & --- & --- \\
 &
 & Specialist
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Contrastive Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Purified Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Contrastive + Purified Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 \cmidrule(lr){2-9}
 & \multirow{5}{*}{\makecell[l]{
Large\\
(\SI{4.98}{\mega\nothing} params.)
}}
 & Generalist
 & 1.0 & 2.0 & --- & --- \\
 &
 & Specialist
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Contrastive Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Purified Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Contrastive + Purified Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 \midrule
\multirow{15}{*}{\makecell[l]{
DPRNN-TasNet}}
 & \multirow{5}{*}{\makecell[l]{
Small\\
(\SI{793}{\kilo\nothing} params.)
}}
 & Generalist
 & 1.0 & 2.0 & --- & --- \\
 &
 & Specialist
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Contrastive Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Purified Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Contrastive + Purified Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
\cmidrule(lr){2-9}
& \multirow{5}{*}{\makecell[l]{
Medium\\
(\SI{1.39}{\mega\nothing} params.)
}}
 & Generalist
 & 1.0 & 2.0 & --- & --- \\
 &
 & Specialist
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Contrastive Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Purified Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Contrastive + Purified Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 \cmidrule(lr){2-9}
& \multirow{5}{*}{\makecell[l]{
Large\\
(\SI{1.98}{\mega\nothing} params.)
}}
 & Generalist
 & 1.0 & 2.0 & --- & --- \\
 &
 & Specialist
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Contrastive Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Purified Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
 &
 & Specialist w/ Contrastive + Purified Loss
 & 1.0 & 2.0 & 3.0 & 4.0 \\
\bottomrule
\end{tabular}
\label{tab:results}
\end{table*}

==> tables/tbl_trainingtime.tex <==
\begin{table}[ht!]
\centering
\caption{Comparison of training time (average \# of examples seen).}
% \begin{tabular}{llll
%     S[table-number-alignment=right, table-format=3.1, round-mode=places, round-precision=1]}
% \toprule
%  \textbf{SSL}
%  & \textbf{FT}
%  & \textbf{\shortstack[l]{Learning\\Rate}}
%  & \textbf{\shortstack[l]{Model\\Size}}
%  & \textbf{\shortstack[l]{Avg. \# of\\Examples}}
%  \\\midrule
%  \multirow{12}{*}{\yes}
%  & \multirow{4}{*}{\SI{0}{\sec}}
%  & \multirow{4}{*}{\num{1e-3}}
%  & Large & \prefix{593907} \\
%  & & & Medium & \prefix{637491} \\
%  & & & Small & \prefix{803578} \\
%  & & & Tiny & \prefix{851408} \\\cmidrule{2-5}
%  & \multirow{4}{*}{\SI{5}{\sec}}
%  & \multirow{4}{*}{\num{1e-4}}
%  & Large & \prefix{5288} \\
%  & & & Medium & \prefix{5716} \\
%  & & & Small & \prefix{6052} \\
%  & & & Tiny & \prefix{6415} \\\cmidrule{2-5}
%  & \multirow{4}{*}{\SI{30}{\sec}}
%  & \multirow{4}{*}{\num{1e-4}}
%  & Large & \prefix{25626} \\
%  & & & Medium & \prefix{26192} \\
%  & & & Small & \prefix{30602} \\
%  & & & Tiny & \prefix{27928} \\\midrule
%  \multirow{12}{*}{\no}
%  & \multirow{4}{*}{\SI{0}{\sec}}
%  & \multirow{4}{*}{\num{1e-3}}
%  & Large & \prefix{1399040} \\
%  & & & Medium & \prefix{1418112} \\
%  & & & Small & \prefix{1388032} \\
%  & & & Tiny & \prefix{1359040} \\\cmidrule{2-5}
%  & \multirow{4}{*}{\SI{5}{\sec}}
%  & \multirow{4}{*}{\num{1e-4}}
%  & Large & \prefix{7882} \\
%  & & & Medium & \prefix{9878} \\
%  & & & Small & \prefix{13430} \\
%  & & & Tiny & \prefix{19277} \\\cmidrule{2-5}
%  & \multirow{4}{*}{\SI{30}{\sec}}
%  & \multirow{4}{*}{\num{1e-4}}
%  & Large & \prefix{39779} \\
%  & & & Medium & \prefix{57533} \\
%  & & & Small & \prefix{57571} \\
%  & & & Tiny & \prefix{81875} \\ 
% \bottomrule
% \end{tabular}
\begin{tabular}{ll
    S[table-number-alignment=right, table-format=3.1, round-mode=places, round-precision=1]
    S[table-number-alignment=right, table-format=3.1, round-mode=places, round-precision=1]
    S[table-number-alignment=right, table-format=3.1, round-mode=places, round-precision=1]
    S[table-number-alignment=right, table-format=3.1, round-mode=places, round-precision=1]}
\toprule
& &
\multicolumn{4}{c}{\textbf{Avg. \# of Examples}} \\
\textbf{\shortstack[l]{Pretraining\\Type}}
& \textbf{\shortstack[l]{Finetuning\\Amount}}
& \text{Tiny}
& \text{Small}
& \text{Medium}
& \text{Large} \\ \midrule
\multirow{3}{*}{Noisy-Target}
& \SI{0}{\sec}
& \prefix{851408}
& \prefix{803579}
& \prefix{637491}
& \prefix{593907} \\
& \SI{5}{\sec}
& \prefix{6415}
& \prefix{6052}
& \prefix{5716}
& \prefix{5288} \\
& \SI{30}{\sec}
& \prefix{27928}
& \prefix{30602}
& \prefix{26192}
& \prefix{25626} \\ \midrule
\multirow{3}{*}{FSL}
& \SI{0}{\sec}
& \prefix{1359040}
& \prefix{1388032}
& \prefix{1418112}
& \prefix{1399040} \\
& \SI{5}{\sec}
& \prefix{19277}
& \prefix{13430}
& \prefix{9878}
& \prefix{7882} \\
& \SI{30}{\sec}
& \prefix{81875}
& \prefix{57571}
& \prefix{57533}
& \prefix{39779} \\
\bottomrule
\end{tabular}
\label{tab:training_time}
\end{table}

==> tables/tbl_waveforms.tex <==
%<*regularse>

%</regularse>

%<*pseudose>

%</pseudose>
